$\mu$DARTS: Model Uncertainty-Aware Differentiable Architecture Search

We present a Model Uncertainty-aware Differentiable ARchiTecture Search ($\mu$DARTS) that optimizes neural networks to simultaneously achieve high accuracy and low uncertainty. We introduce concrete dropout within DARTS cells and include a Monte-Carlo regularizer within the training loss to optimize the concrete dropout probabilities. A predictive variance term is introduced in the validation loss to enable searching for architecture with minimal model uncertainty. The experiments on CIFAR10, CIFAR100, SVHN, and ImageNet verify the effectiveness of $\mu$DARTS in improving accuracy and reducing uncertainty compared to existing DARTS methods. Moreover, the final architecture obtained from $\mu$DARTS shows higher robustness to noise at the input image and model parameters compared to the architecture obtained from existing DARTS methods.

==> tex/BroaderImpact.tex <==
\section*{Broader Impact}
% Uncertainty estimation of neural networks is a critical challenge for many practical application\cite{gal2016uncertainty, kendall2017uncertainties, kendall2015bayesian}. The uncertainty of a neural network can be approximated by incorporating Monte-Carlo dropout \cite{gal2015dropout}. Gal et. al. used concrete dropout as a continuous relaxation of dropout’s discrete masks to improve accuracy and provide better uncertainty calibration ~\cite{gal2017concrete}. For a given training dataset, the model uncertainty of a network depends on its architecture. However, there is no prior work that aims to optimize network architectures to reduce model uncertainty as well as improve accuracy.


%This paper develops a methodology to seek neural network architecture that simultaneously improves accuracy and reduces model uncertainty. 
% We approach this problem by exploring neural architecture search (NAS)~\cite{bender2019understanding, baker2016designing, bergstra2013making, zoph2016neural,real2019aging}. %The NAS methods for automatically searching for architectures with high performance (accuracy) have demonstrated success in computer vision tasks\cite{zoph2016neural, real2019aging}. More recently, 
% Liu et al. have proposed differentiable architecture search (DARTS) ~\cite{liu2018darts} that uses continuous relaxation of the architecture representation allowing efficient search of the architecture using gradient descent, thereby improving the efficiency of NAS.
% The DARTS perform a bi-level optimization problem where an outer loop searches over architectures using a validation loss ($\mathcal{L}_{\text {valid}}$) and the inner loop optimizes parameters (weights) for each architecture using a training loss ($\mathcal{L}_{\text {train}}$). 

% We advance the baseline DARTS framework by introducing: (a) concrete dropout ~\cite{gal2017concrete} layers within DARTS cell to enable uncertainty estimation; (b) a Monte-Carlo dropout based regularizer ~\cite{gal2015dropout} within $\mathcal{L}_{\text {train}}$ to optimize dropout probabilities; and (c) a predictive variance term in $\mathcal{L}_{\text {valid}}$ to search for architecture with minimal model uncertainty. This paper makes following key contributions:
% \begin{itemize}
%     \item We develop the UDARTS framework and training process to simultaneously improve accuracy and reduce model uncertainty of neural network.  
%     \item We prove that UDARTS reduces eigenvalues of the Hessian matrix of the validation loss thereby generating a more robust neural architecture with a better generalization performance than the ones obtained with baseline DARTS.
%     \item We experimentally demonstrate that UDARTS improves the robustness of the neural architecture search method as well as the enhances accuracy, uncertainty, and robustness of the final architecture found using the architecture search.
% \end{itemize}

%The experimental results on CIFAR10 and CIFAR100 shows the UDARTS generates network with $99\%$ accuracy and $0.09$ model uncertainty, while baseline DARTS only enable $90\%$ accuracy with $0.12$ uncertainty. 

%  We further prove that UDARTS reduces eigenvalues of the Hessian matrix of the validation loss, thereby generating a more robust neural architecture with a better generalization performance than the ones obtained with baseline DARTS.


% Recently, there has been a growing interest in developing algorithmic solutions to automate the manual process of architecture design.  

% Thus, in this paper, we aim to leverage this DARTS approach to find the best possible architecture from the architecture search space which not only increases the accuracy but also minimizes the uncertainty of the model.


% As the estimated uncertainty estimate 

% Coupled with a modified optimisation objective, this technique allows for the selection of an optimal dropout probability in large models, and thus resulting in faster experimentation cycles.

Model uncertainty of neural networks has emerged as a key challenge that provides a measure of how certain a model is about the prediction that it is making.
In the last couple of years, calculating the model uncertainty of a deep learning model has captured the interest of many researchers. Model uncertainty is an important metric as it quantifies the times when the model gives overconfident predictions which may turn out to be critical in certain scenarios. With model confidence, we can treat uncertain inputs and special cases explicitly. For example in the case of a self-driving car, the predictions are of extremely high importance as it takes life-critical decisions based on the output of the classifiers and object detectors. Such a situation may arise when suppose the classifier could not detect an individual on the road. Without a measure of uncertainty, the decision system may give erroneous outputs which may lead to unwanted outcomes. On the other hand, the uncertainty measures act as a safety net which can enable the system to take into account the inputs from a different sensor. Calculating the uncertainty and getting an architecture that minimizes the uncertainty of the model thus plays a key role in the future of neural network modeling. With each day, we are more reliant on learning models, and thus it has become imperative that the model also knows what it does not know.
% Model uncertainty is a function of the model used.

% However, though the present work determines the model uncertainty for a given architecture, there has been no current work that tries to find an architecture that minimizes the model uncertainty. 

==> tex/Tables.tex <==
\begin{table*}[]
\centering
\caption{Accuracy and Uncertainty of Final DNN Models from Neural Architecture Search Processes}
\label{tab:acc_unc}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{c||c||c c||c c||c c||c c}
\hline \hline
\textbf{Model} & \textbf{FLOPS}(M) & \multicolumn{2}{c||}{\textbf{CIFAR10}} & \multicolumn{2}{c||}{\textbf{CIFAR100}} & \multicolumn{2}{c||}{\textbf{SVHN}}& \multicolumn{2}{c}{\textbf{ImageNet}} \\ 
\multicolumn{1}{l||}{} & & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l||}{Uncertainty} & \multicolumn{1}{l}{Accuracy} & \multicolumn{1}{l||}{Uncertainty} & \multicolumn{1}{l}{Accuracy} & Uncertainty & \multicolumn{1}{l}{Accuracy} & Uncertainty \\ \hline \hline
\textbf{MobileNetv2}$\dagger$ & 569 & 88.51 & 0.915 & 68.54 & 1.266 & 93.67 & 0.247 & 67.83 & 1.853     \\ %\hline
\textbf{VGG16}$\dagger$ & 160 & 84.11 & 1.034 & 71.19 & 1.482 & 93.15 &  0.344 & 61.46 & 1.897   \\ %\hline
\textbf{ResNet20}$\dagger$ & 320 & 86.47 & 0.985 & 75.22 & 1.346 & 93.74 &  0.288  & 64.11 & 1.846  \\ %\hline
\textbf{EfficientNet-B0}$\dagger$ & 390 & 88.01  & 0.899 & 76.02  & 0.915 & 94.87 &  0.251  & 69.83 & 1.833  \\ \hline \hline
\textbf{DARTS}$\dagger$& 595 & 92.4 & N/A & 76.33 & N/A & 95.00 & N/A  & 72.36 & NA   \\ %\hline
\textbf{DARTS-CD}& 598 & 93.159 & 0.209 & 76.91 & 0.558 & 95.15 & 0.092  & 73.52 & 1.693   \\ %\hline
\textbf{RDARTS-CD}& 605 & 94.026   & 0.186  &  77.15  & 0.509  &  95.48 &  0.07  & 73.77 & 1.685  \\ \hline \hline
\begin{tabular}[c]{@{}c@{}}$\mu$\textbf{DARTS} \\ (This Work)\end{tabular}& 602 & 96.723 & 0.089 & 80.61 & 0.361 & 96.76 & 0.026  & 78.76 & 1.523   \\ \hline \hline
\end{tabular}%
 }
\end{table*}


==> tex/extra.tex <==
\section{Concrete Dropout in DARTS search space}
DARTS optimization procedure is defined as a bi-level optimization problem where $\mathcal{L}_{\text {valid}}$ is the outer objective  and $\mathcal{L}_{\text {train}}$ is the inner objective as:
$$
\begin{array}{l}
\min _{\alpha} \mathcal{L}_{v a l i d}\left(\alpha, w^{*}(\alpha)\right) \\
\text { s.t. } \quad w^{*}(\alpha)={\arg \min }_{w} \mathcal{L}_{\text {train}}(\alpha, w)
\end{array}
$$
where both losses are determined by both the architecture parameters $\alpha$ (outer variables) and the network weights $w$ (inner variables). 
Now, sine our objective is to minimze the uncertainty using the neural architecture search, and since the validation loss optimizes the architecture parameter, we add with it the model's predictive variance. Similarly, since the training loss optimizes the network weights, we include the monte carlo dropout loss function to it. Thus, our bi-level optimization function is transformed to:
\begin{align}
&\min _{\alpha} \mathcal{L}_{v a l i d}\left(\alpha, w^{*}(\alpha)\right) + \operatorname{Var}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right) \\
\text { s.t. } \quad w^{*}(\alpha)&={\arg \min }_{w} \mathcal{L}_{\text {train}}(\alpha, w) + \widehat{\mathcal{L}}_{\mathrm{MC}}(\theta)
\end{align}

where the model's predictive variance is given by: 

\begin{equation}
\operatorname{Var}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right) \approx \tau^{-1} \mathbf{I}_{D} +\frac{1}{T} \sum_{t=1}^{T} \widehat{\mathbf{y}}^{*}\left(\mathbf{x}^{*}, \mathbf{W}_{1}^{t}, \ldots, \mathbf{W}_{L}^{t}\right)^{T} \widehat{\mathbf{y}}^{*}\left(\mathbf{x}^{*}, \mathbf{W}_{1}^{t}, \ldots, \mathbf{W}_{L}^{t}\right) \\
-\mathbb{E}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right)^{T} \mathbb{E}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right)
\end{equation}

and the monte carlo dropout loss is given as:

\begin{align}
\widehat{\mathcal{L}}_{\mathrm{MC}}(\theta) &=-\frac{1}{M} \sum_{i \in S} \log p\left(\mathbf{y}_{i} |\mathbf{f}^{\omega}\left(\mathbf{x}_{i}\right)\right)+\frac{1}{N} \mathrm{KL}\left(q_{\theta}(\omega) \| p(\omega)\right) \\
&= -\frac{1}{M} \sum_{i \in S} \log p\left(\mathbf{y}_{i} | \mathbf{f}^{\omega}\left(\mathbf{x}_{i}\right)\right) +\frac{1}{N} \sum_{l=1}^{L} \frac{l^{2}(1-p)}{2}\|\mathbf{M}\|^{2}-K \mathcal{H}(p)
\end{align}

The total derivative of $\mathcal{L}_{\text {valid}}$ w.r.t. $\alpha$ evaluated on $\left(\alpha, w^{*}(\alpha)\right)$ would be:
$$
\frac{d}{d \alpha} (( \mathcal{L}_{v a l i d} + \operatorname{Var}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right) ))=\nabla_{\alpha} \mathcal{L}_{v a l i d}-\nabla_{w} \mathcal{L}_{v a l i d}\left(\nabla_{w}^{2} \mathcal{L}_{t r a i n}\right)^{-1} \nabla_{\alpha, w}^{2} \mathcal{L}_{t r a i n} + \nabla_{\alpha}
$$
where $\nabla_{\alpha}=\frac{\partial}{\partial \alpha}, \nabla_{w}=\frac{\partial}{\partial w}$ and $\nabla_{\alpha, w}^{2}=\frac{\partial^{2}}{\partial \alpha \partial w} .$ 




















Given the outer objective function $F: \mathbb{R}^{P} \times \mathbb{R}^{N} \rightarrow \mathbb{R}$ and the inner objective function $f: \mathbb{R}^{P} \times \mathbb{R}^{N} \rightarrow \mathbb{R},$ the bi-level optimization problem is given by
$$
\begin{array}{l}
\min _{y \in \mathbb{R}^{P}} F\left(y, \theta^{*}(y)\right) \\
\text { s.t. } \quad \theta^{*}(y) \in \underset{\theta \in \mathbb{R}^{N}}{\arg \min } f(y, \theta)
\end{array}
$$
where $y \in \mathbb{R}^{P}$ and $\theta \in \mathbb{R}^{N}$ are the outer and inner variables, respectively. One may also see the bi-level problem as a constrained optimization problem, with the inner problem as a constraint.
In general, even in the case when the inner objective is strongly convex and has an unique minimizer $\theta^{*}(y)=\arg \min _{\theta \in \mathbb{R}^{N}} f(y, \theta),$ it is not possible to directly optimize the outer objective.

\textbf{Continuous relaxation of the search space.} In agreement with prior work (Zoph et all, 2018 ; Real et al., 2019), DARTS optimizes only substructures called cells that are stacked to define the full network architecture. Each cell contains $N$ nodes organized in a directed acyclic graph. The graph contains two inputs nodes (given by the outputs of the previous two cells), a set of intermediate nodes, and one output node (given by concatenating all intermediate nodes). Each intermediate node $x^{(j)}$ represents a feature map. 

Instead of applying a single operation to a specific node during architecture search, DARTS relax the decision which operation to choose by computing the intermediate node as a mixture of candidate operations,
applied to predecessor nodes 

$$x^{(i)}, i<j, x^{(j)}=\sum_{i<j} \sum_{o \in \mathcal{O}} \frac{\exp \left(\alpha_{s}^{i, j}\right)}{\sum_{o^{\prime}} \epsilon O \exp \left(\alpha_{o^{\prime}, \bar{\prime}}^{(i)}\right.} o\left(x^{(i)}\right),$$ 

where $\mathcal{O}$ denotes the set of all candidate operations (e.g., $3 \times 3$ convolution, skip connection, $3 \times 3$ max pooling, etc.) and $\alpha=\left(\alpha_{o}^{i, j}\right)_{i, j, o}$ serves as a real-valued parameterization of the architecture.

\textbf{Gradient-based optimization of the search space.} DARTS then optimizes both the weights of the search network (often called the weight-sharing or one-shot model, since the weights of all individual subgraphs/architectures are shared) and architectural parameters by alternating gradient descent. 

The network weights and the architecture parameters are optimized on the training and validation set, respectively. This can be interpreted as solving the bi-level optimization problem where $F$ and $f$ are the validation and training loss, $\mathcal{L}_{\text {valid}}$ and $\mathcal{L}_{\text {train}},$ respectively, while $y$ and $\theta$ denote the architectural parameters $\alpha$ and network weights $w$, respectively. Note that DARTS only approximates the lower-level solution by a single gradient step. At the end of the search phase, a discrete cell is obtained by choosing the $k$ most important incoming operations for each intermediate node while all others are pruned. Importance is measured by the operation weighting factor $$\frac{\exp \left(\alpha_{o}^{i, j}\right)}{\sum_{o^{\prime} \in O} \exp\left(\alpha_{\alpha^{\prime}}^{2, j}\right)}$$


\textbf{Theorem:}   
DARTS optimization procedure is defined as a bi-level optimization problem where $\mathcal{L}_{\text {valid}}$ is the outer objective  and $\mathcal{L}_{\text {train}}$ is the inner objective as:
$$
\begin{array}{l}
\min _{\alpha} \mathcal{L}_{v a l i d}\left(\alpha, w^{*}(\alpha)\right) \\
\text { s.t. } \quad w^{*}(\alpha)={\arg \min }_{w} \mathcal{L}_{\text {train}}(\alpha, w)
\end{array}
$$
where both losses are determined by both the architecture parameters $\alpha$ (outer variables) and the network weights $w$ (inner variables). 
Now, sine our objective is to minimze the uncertainty using the neural architecture search, and since the validation loss optimizes the architecture parameter, we add with it the model's predictive variance. Similarly, since the training loss optimizes the network weights, we include the monte carlo dropout loss function to it. Thus, our bi-level optimization function is transformed to:


\begin{equation}
\min _{\alpha} \mathcal{L}_{v a l i d}\left(\alpha, w^{*}(\alpha)\right) + \operatorname{Var}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right) \\
\text { s.t. } \quad w^{*}(\alpha)={\arg \min }_{w} \mathcal{L}_{\text {train}}(\alpha, w) + \widehat{\mathcal{L}}_{\mathrm{MC}}(\theta)
\end{equation}

where the model's predictive variance is given by: 

\begin{equation}
\operatorname{Var}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right) \approx \tau^{-1} \mathbf{I}_{D} +\frac{1}{T} \sum_{t=1}^{T} \widehat{\mathbf{y}}^{*}\left(\mathbf{x}^{*}, \mathbf{W}_{1}^{t}, \ldots, \mathbf{W}_{L}^{t}\right)^{T} \widehat{\mathbf{y}}^{*}\left(\mathbf{x}^{*}, \mathbf{W}_{1}^{t}, \ldots, \mathbf{W}_{L}^{t}\right) \\
-\mathbb{E}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right)^{T} \mathbb{E}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right)
\end{equation}

and the monte carlo dropout loss is given as:

\begin{align}
\widehat{\mathcal{L}}_{\mathrm{MC}}(\theta) &=-\frac{1}{M} \sum_{i \in S} \log p\left(\mathbf{y}_{i} |\mathbf{f}^{\omega}\left(\mathbf{x}_{i}\right)\right)+\frac{1}{N} \mathrm{KL}\left(q_{\theta}(\omega) \| p(\omega)\right) \\
&= -\frac{1}{M} \sum_{i \in S} \log p\left(\mathbf{y}_{i} | \mathbf{f}^{\omega}\left(\mathbf{x}_{i}\right)\right) +\frac{1}{N} \sum_{l=1}^{L} \frac{l^{2}(1-p)}{2}\|\mathbf{M}\|^{2}-K \mathcal{H}(p)
\end{align}

The total derivative of $\mathcal{L}_{\text {valid}}$ w.r.t. $\alpha$ evaluated on $\left(\alpha, w^{*}(\alpha)\right)$ would be:
$$
\frac{d}{d \alpha} (( \mathcal{L}_{v a l i d} + \operatorname{Var}_{q\left(\mathbf{y}^{*} | \mathbf{x}^{*}\right)}\left(\mathbf{y}^{*}\right) ))=\nabla_{\alpha} \mathcal{L}_{v a l i d}-\nabla_{w} \mathcal{L}_{v a l i d}\left(\nabla_{w}^{2} \mathcal{L}_{t r a i n}\right)^{-1} \nabla_{\alpha, w}^{2} \mathcal{L}_{t r a i n} + \nabla_{\alpha}
$$
where $\nabla_{\alpha}=\frac{\partial}{\partial \alpha}, \nabla_{w}=\frac{\partial}{\partial w}$ and $\nabla_{\alpha, w}^{2}=\frac{\partial^{2}}{\partial \alpha \partial w} .$ 


%Computing the inverse of the Hessian is in general not possible considering the high dimensionality of the model parameters $w$, therefore resolving to gradient-based iterative algorithms for finding $w^{*}$ is necessary. However, this would also require to optimize the model parameters $w$ till convergence each time $\alpha$ is updated. If our model is a deep neural network it is clear that this computation is expensive, therefore Liu et al. (2019) propose to 
We approximate $w^{*}(\alpha)$ by updating the current model parameters $w$ using a single gradient descent step:
$$
w^{*}(\alpha) \approx w-\xi \nabla_{w} \mathcal{L}_{t r a i n}(\alpha, w)
$$
where $\xi$ is the learning rate for the virtual gradient step DARTS takes with respect to the model weights $w$. The gradient of  $ w^{*}(\alpha)$  with respect to $\alpha$  is
$$
\frac{\partial w^{*}}{\partial \alpha}(\alpha)=-\xi \nabla_{\alpha, w}^{2} \mathcal{L}_{t r a i n}(\alpha, w)
$$

\noindent\makebox[\linewidth]{\rule{\paperwidth}{0.4pt}}

By setting the evaluation point $w^{*}=w-\xi \nabla_{w} \mathcal{L}_{\text {train}}(\alpha, w)$ and following the same derivation as in Appendix $[\text { A. } .1]$ we obtain the DARTS architectural gradient approximation:
$$
\frac{d \mathcal{L}_{\text {valid}}}{d \alpha}(\alpha)=\nabla_{\alpha} \mathcal{L}_{\text {valid}}\left(\alpha, w^{*}\right)-\xi \nabla_{w} \mathcal{L}_{\text {valid}}\left(\alpha, w^{*}\right) \nabla_{\alpha, w}^{2} \mathcal{L}_{\text {train}}\left(\alpha, w^{*}\right)
$$
where the inverse Hessian $\nabla_{w}^{2} \mathcal{L}_{t r a i n}^{-1}$ in (9) is replaced by the learning rate $\xi$. This expression however contains again an expensive vector-matrix product. Liu et al. (2019) reduce the complexity by using the finite difference approximation around $w^{\pm}=w \pm \epsilon \nabla_{w} \mathcal{L}_{\text {valid}}\left(\alpha, w^{*}\right)$ for some small
$\epsilon=0.01 /\left\|\nabla_{w} \mathcal{L}_{v a l i d}\left(\alpha, w^{*}\right)\right\|_{2}^{17}$ to compute the gradient of $\nabla_{\alpha} \mathcal{L}_{t r a i n}\left(\alpha, w^{*}\right)$ with respect to $w$ as
$$
\begin{array}{c}
\nabla_{\alpha, w}^{2} \mathcal{L}_{t r a i n}\left(\alpha, w^{*}\right) \approx \frac{\nabla_{\alpha} \mathcal{L}_{t r a i n}\left(\alpha, w^{+}\right)-\nabla_{\alpha} \mathcal{L}_{t r a i n}\left(\alpha, w^{-}\right)}{2 \epsilon \nabla_{w} \mathcal{L}_{v a l i d}\left(\alpha, w^{*}\right)} \\
\nabla_{w} \mathcal{L}_{v a l i d}\left(\alpha, w^{*}\right) \nabla_{\alpha, w}^{2} \mathcal{L}_{t r a i n}\left(\alpha, w^{*}\right) \approx \frac{\nabla_{\alpha} \mathcal{L}_{t r a i n}\left(\alpha, w^{+}\right)-\nabla_{\alpha} \mathcal{L}_{t r a i n}\left(\alpha, w^{-}\right)}{2 \epsilon}
\end{array}
$$
In the end, combining equation $[12 \text { and equation }[\mathbb{Z}\text { gives the gradient to compute the architectural }$ updates in DARTS:
$$
\frac{d \mathcal{L}_{\text {valid}}}{d \alpha}(\alpha)=\nabla_{\alpha} \mathcal{L}_{\text {valid}}\left(\alpha, w^{*}\right)-\frac{\xi}{2 \epsilon}\left(\nabla_{\alpha} \mathcal{L}_{\text {train}}\left(\alpha, w^{+}\right)-\nabla_{\alpha} \mathcal{L}_{\text {train}}\left(\alpha, w^{-}\right)\right)
$$
In all our experiments we always use $\xi=\eta$ (also called second order approximation in Liu et al.
(2019)), where $\eta$ is the learning rate used in SGD for updating the parameters $w$







######################################################
Proof:

Now for the case of UDARTS, we add the predictive variance term to the DARTS validation loss. 

\begin{comment}


%$(Y-\bar{Y})^{T}(Y-\bar{Y}) = Y^{T}Y - Y^{T}\bar{Y}- \bar{Y}^{T}Y + \bar{Y}^{T}\bar{Y}$
\begin{align}
\operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha})&=\frac{1}{T} \sum_{i=1}^{T}\left(\mathbf{y}_{i} - \sigma(\operatorname{model}\left(\mathbf{x}_{i}, \mathbf{\alpha}\right)\right))^{2}\\
&=\frac{1}{T} \sum_{i=1}^{T}\left(\mathbf{y}_{i} - \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})\right)^{2} \quad [\text{Using linear model}]
\end{align}
where $\left\{\mathbf{y}_{i}\right\}_{t=1}^{T}$ is a set of $T$ sampled outputs for weights instances $\omega^{i} \sim q(\omega ; \Phi)$ and $\mathbf{y}=1 / T \sum_{i} \mathbf{y}_{i}$. 
\begin{align}
\nabla_{\alpha} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= -\frac{2}{T} \sum_{i=1}^{T}\left(\mathbf{y}_{i} - \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})\right)\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1-\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))\mathbf{x}_{i}\\
\nabla_{\alpha}^{2} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= - \frac{2}{T} \sum_{i=1}^{T} [-\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1-\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) +  \left(\mathbf{y}_{i} - \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})\right)\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1-\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}  \\ & - (\mathbf{y}_{i} - \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}(1-\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))]  \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
\end{align}

Thus, we get that the spectral radius of the hessian as 
\begin{align}
    \nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}} &= \frac{1}{N} \sum_{i=1}^{N} \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1-\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) \mathbf{x}_{i} \mathbf{x}_{i}^{T} - \frac{2}{N} \sum_{i=1}^{N}  \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
    %&= \frac{1}{N} \sum_{i=1}^{N} (\sigma_{i}\mathbf{x}_{i} \mathbf{x}_{i}^{T} - 2\mathbf{x}_{i} \mathbf{x}_{i}^{T}) \\
    &= \frac{(\sigma_{i}-2)}{N} \sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}
\end{align}

Thus, the spectral radius is given as:
\begin{align}
    \rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}}) &= \frac{(\sigma_{i}-2)}{N} \sum_{i=1}^{N} \| \mathbf{x}_{i} \mathbf{x}_{i}^{T} \|_{2}^{2} \\
    & \le -\frac{7}{4N} \sum_{i=1}^{N} \| \mathbf{x}_{i} \mathbf{x}_{i}^{T} \|_{2}^{2} \\
    & \le \rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}})
\end{align}

Thus, the spectral radius of the UDARTS method is smaller than the spectral radius of DARTS.


\begin{align}
\operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha})&=\frac{1}{T} \sum_{i=1}^{T} \sigma\left(f^{\tilde{\alpha}_{t}}\left(x^{*}\right)\right) \\
&= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}) \\
\nabla_{\alpha} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})) \mathbf{x}_{i} \\
\nabla_{\alpha}^{2} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))[1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})]\mathbf{x}_{i}\mathbf{x}_{i}^{T} \\
&= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))[1- 2\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})]\mathbf{x}_{i}\mathbf{x}_{i}^{T} \\
\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} &= \frac{1}{N} \sum_{i=1}^{N} \sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T} + \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))[1- 2\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})]\mathbf{x}_{i}\mathbf{x}_{i}^{T} \\
&= \frac{1}{N} \sum_{i=1}^{N} \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)\left(\mathbf{x}_{i}^{T} \mathbf{z}\right) \\
&=\frac{1}{N} \sum_{i=1}^{N} \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2} +  \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))[1- 2\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})]\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2}
\end{align}
For the problem, we choose the number of samples $T$ equal to the cardinality of the dataset $N$. Thus, the equation simplifies to 
\begin{align}
    \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} &= \frac{1}{N} \sum_{i=1}^{N} \{\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})) + \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))[1- 2\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})]\}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2}
\end{align}


Since the sigmoid function outputs value in the region of $[0,1]$, we can show that $\exists x_{1}, x_{2} , 0 \le x_{1} \le x \le x_{2} \le 1$ such that \[\rho(\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})) + \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))[1- 2\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})]) < \rho(\sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\tilde{\alpha}}))\]

\end{comment}


\begin{align}
\operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha})
&= \frac{1}{T} \sum_{i=1}^{T}\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) - (\frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}\\
\nabla_{\alpha} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) 2\mathbf{\alpha}^{T}\mathbf{x}_{i} -  \frac{2}{T^{2}} \sum_{i=1}^{T} \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}) (1 - \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) \mathbf{x}_{i}\\
\nabla_{\alpha}^{2} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= \frac{1}{T} \sum_{i=1}^{T} \{ [\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -2(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))]2\alpha^{T}\alpha \mathbf{x}_{i}\mathbf{x}^{T}_{i} \nonumber\\ &+ \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) 2\mathbf{x}_{i}\mathbf{x}^{T}_{i} \} \nonumber\\ &- \frac{2}{T^{2}} \sum_{i=1}^{T} \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) -2(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
% &= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))[1- 2\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})]\mathbf{x}_{i}\mathbf{x}_{i}^{T} \\
\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} &= \frac{1}{N} \sum_{i=1}^{N} \sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T} + \nonumber\\ &\frac{1}{T} \sum_{i=1}^{T} \{ [\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -2(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))]2\alpha^{T}\alpha \mathbf{x}_{i}\mathbf{x}^{T}_{i} \nonumber\\ &+ \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) 2\mathbf{x}_{i}\mathbf{x}^{T}_{i} \} \nonumber\\ &+ \frac{2}{T^{2}} \sum_{i=1}^{T} -\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) +2(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) \mathbf{x}_{i} \mathbf{x}_{i}^{T}
\end{align}

Since we can choose the number of samples $T$, without loss of generality, let us consider the case when $T=N$.
Again, since the softmax is a convex function, we can use Jensen's inequality as \[ (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2} \le \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})\]

Therefore the hessian simplifies to the following form:
\begin{align}
\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} &\le  \frac{1}{T} \sum_{i=1}^{T} [\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)  + \nonumber \\ & \{ [\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -4(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))]\alpha^{T}\alpha \nonumber\\ &+ 2\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))  \} \nonumber\\ &- 2 \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) +4(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))] \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
 &\le  \frac{1}{T} \sum_{i=1}^{T} [\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)  + \nonumber\\ & \{ [(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2}(1- (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2}) -4(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2}(1- (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2})]\alpha^{T}\alpha \nonumber\\ &+ 2(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^2(1 - (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^2)  \} \nonumber\\ &+ 2 \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) -4(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))] \mathbf{x}_{i} \mathbf{x}_{i}^{T} 
\end{align}

Treating this equation as a polynomial in $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})$ such that the values of $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}) \in [0,1]$, we get the following polynomial: \[f(x) = (4\alpha^2 -3)x^4 -4x^3 +(8-4\alpha^2)x^2 -x\] such that \[f(x) \le x(1-x)\] for $x \in [0,1]$. Hence we may say that the spectral radius of the hessian of the UDARTS are smaller than the ones of the DARTS method






##################################################
Proof Iter 2



We aim to prove that the inclusion of the predictive variance improves the performance of the UDARTS method compared to normal DARTS and will search for a flatter minima.
In order to prove this, we aim to show that the spectral radius of the Hessian of the validation loss $\rho(\nabla_{\alpha}^2 \mathcal{L}_{\text{valid}})$ is smaller than the spectral radius of the normal DARTS method.  First of all we consider the cross entropy loss which is used to calculate the basic validation loss $\mathcal{L}_{\text{valid}}$. 
The gradient and the corresponding hessian of the cross entropy loss are given as follows:
\begin{equation}g(\mathbf{\alpha})=-\frac{1}{N} \sum_{i=1}^{N} y_{i} \log \left(\sigma\left(\operatorname{model}\left(\mathbf{x}_{i}, \mathbf{\alpha}\right)\right)\right)+\left(1-y_{i}\right) \log \left(1-\sigma\left(\operatorname{model}\left(\mathbf{x}_{i}, \mathbf{\alpha}\right)\right)\right)\end{equation}

For this proof we consider a linear model given as $\operatorname{model}\left(\mathbf{x}_{i}, \mathbf{\alpha}\right)=\mathbf{x}_{i}^{T} \mathbf{\alpha}$

\begin{equation}\nabla_{\alpha} g(\mathbf{\alpha})=-\frac{1}{N} \sum_{i=1}^{N}\left(y_{i}-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i}\end{equation}

\begin{equation}\nabla_{\alpha}^{2} g(\mathbf{\alpha})=\frac{1}{N} \sum_{i=1}^{N} \sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T}\end{equation}

Now, in order to prove that the cross entropy function is convex, we prove that the hessian is positive semi-definite. We know that the smallest eigenvalue of any square symmetric matrix is given as the minimum of the Rayleigh quotient, i.e., the smallest value taken by

\[
\mathbf{z}^{T} \nabla_{\alpha}^{2} g(\mathbf{\alpha}) \mathbf{z}
\]
for any unit-length vector $\mathbf{z}$ and any possible weight vector $\mathbf{\alpha}$. Substituting in the particular form of the Hessian here, denoting $\sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)$ for each $i$ for short, we have
\begin{equation}
\mathbf{z}^{T} \nabla_{\alpha}^{2} g(\mathbf{\alpha}) \mathbf{z}=\mathbf{z}^{T}\left(\frac{1}{N} \sum_{i=1}^{N} \sigma_{i} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)\left(\mathbf{x}_{i}^{T} \mathbf{z}\right)=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2}
\end{equation}
since it is always the case that $\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2} \geq 0$ and $\sigma_{i} \geq 0,$ it follows that the smallest value the above can take is 0 meaning that this is the smallest possible eigenvalue of the softmax cost's Hessian. since this is the case, the softmax
cost must be convex.
We know that for a matrix $A$, 
\begin{equation}\|A\|_{2}^{2}=\max _{x \neq 0} \frac{\|A x\|_{2}^{2}}{\|x\|_{2}^{2}}=\max _{x \neq 0} \frac{x^{T} A^{T} A x}{x^{T} x}=\lambda_{\max }\left(A^{T} A\right)=\rho\left(A^{T} A\right)\end{equation}



Building on the analysis above showing that the cross-entropy cost is convex, we can likewise compute its largest possible eigenvalue by noting that $\sigma_{i} \le \frac{1}{4}$. Thus the largest value the Rayleigh quotient can take is bounded above for any $\mathbf{z}$ as
\[
\mathbf{z}^{T} \nabla_{\alpha}^{2} g(\mathbf{\alpha}) \mathbf{z} \leq \frac{1}{4 N} \mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}
\]
since the maximum value $\mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}$ can take is the maximum eigenvalue of the matrix $\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T},$ thus the spectral radius for the Cross Entropy cost is given as
\[
\rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = \frac{1}{4 N}\left\|\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right\|_{2}^{2}
\]

Now for the case of UDARTS, we add the predictive variance term to the DARTS validation loss. 



\begin{align}
\operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha})
&= \frac{1}{T} \sum_{i=1}^{T}\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) - \frac{1}{T}( \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2}\\
\nabla_{\alpha} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) 2\mathbf{\alpha}^{T}\mathbf{x}_{i} -  \frac{2}{T} \sum_{i=1}^{T} (\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^2 (1 - \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) \mathbf{x}_{i}\\
\nabla_{\alpha}^{2} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= \frac{1}{T} \sum_{i=1}^{T} \{ [\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -2(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))]4\alpha^{T}\alpha \mathbf{x}_{i}\mathbf{x}^{T}_{i} \nonumber\\ &+ \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) 2\mathbf{x}_{i}\mathbf{x}^{T}_{i} \} \nonumber\\ &- \frac{2}{T} \sum_{i=1}^{T} 2(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^2(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) -3(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{3}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
% &= \frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))[1- 2\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})]\mathbf{x}_{i}\mathbf{x}_{i}^{T} \\
\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} &= \frac{1}{N} \sum_{i=1}^{N} \sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T} + \nonumber\\ &\frac{1}{T} \sum_{i=1}^{T} \{ [\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -2(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))]4\alpha^{T}\alpha \mathbf{x}_{i}\mathbf{x}^{T}_{i} \nonumber\\ &+ \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) 2\mathbf{x}_{i}\mathbf{x}^{T}_{i} \} \nonumber\\ &- \frac{2}{T} \sum_{i=1}^{T} 2(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^2 (1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) -3(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{3}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) \mathbf{x}_{i} \mathbf{x}_{i}^{T}
\end{align}

Since we can choose the number of samples $T$, without loss of generality, let us consider the case when $T=N$.
Again, since the softmax is a convex function, we can use Jensen's inequality as \[ (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2} \le \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})\]

Therefore the hessian simplifies to the following form:
\begin{align}
\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} &=  \frac{1}{T} \sum_{i=1}^{T} [\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)  + \nonumber \\ & \{ [4\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -8(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))]\alpha^{T}\alpha \nonumber\\ &+ 2\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))  \} \nonumber\\ &- 4 (\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^2(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) +6(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{3}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))] \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
 &\ge  \frac{1}{T} \sum_{i=1}^{T} [\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)  + \nonumber\\ & \{ [4(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2}(1- (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2}) -8(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{4}(1- (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^{2})]\alpha^{T}\alpha \nonumber\\ &+ 2(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^2(1 - (\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right))^2)  \} \nonumber\\ &-4 (\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^2(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) +6(\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{3}(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))] \mathbf{x}_{i} \mathbf{x}_{i}^{T} 
\end{align}

Treating this equation as a polynomial in $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})$ such that the values of $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}) \in [0,1]$, we get the following polynomial: \[f(x) = (4\alpha^2 -3)x^4 -4x^3 +(8-4\alpha^2)x^2 -x\] such that \[f(x) \le x(1-x)\] for $x \in [0,1]$. Hence we may say that the spectral radius of the hessian of the UDARTS are smaller than the ones of the DARTS method

==> tex/robustness.tex <==
\section{UDARTS and Flat Minima}
\label{sec:robust}

In this section, we prove that the eigenvalue of the Hessian of validation loss in UDARTS ($\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}}$) is lower than the eigenvalue of the Hessian of validation loss in DARTS ($\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$). 


\begin{lemma}
The largest eigenvalue of the Hessian of the validation loss of DARTS is given by, \begin{equation}
    \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = \frac{\max \sigma_i}{N}\lambda_{\max} (\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T})
\end{equation} 

where \begin{equation}
     \sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \nonumber
\end{equation}
\label{lemma:DARTS}
\end{lemma}


\textbf{Corollary.}  The validation loss function of the standard DARTS ($\mathcal{L}_{\text{valid}}^{\text{DARTS}}$) method is convex in nature.


\begin{lemma}
The largest eigenvalue of the Hessian of the validation loss of UDARTS is given by, \begin{equation}
    \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}}) \le \frac{ \sigma_{ud}^{max}}{N}\lambda_{\text{max}}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) 
\end{equation}  
where
\begin{flalign*} 
\sigma_{ud} &= \sqrt{\sigma_{x^2}}\left(1-\sqrt{\sigma_{x^2}}\right)  +  4\alpha^2 \sigma_{x^2}(1- \sigma_{x^2}) \nonumber \\ &-8\alpha^2(\sigma_{x^2})^{2}(1- \sigma_{x^2}) 
 + 2\sigma_{x^2}(1 - \sigma_{x^2})  \nonumber\\
 &-2(\sqrt{\sigma_{x^2}}(1-\sqrt{\sigma_{x^2}})+ \sqrt{\sigma_{x^2}}) \nonumber \\
 \sigma_{x^2} &= \sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) \text{ and } \sigma_{x} = \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})  \nonumber
\end{flalign*}



\label{lemma:UDARTS}
\end{lemma}



\begin{lemma}
If $\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}})$ and $\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})$ be the maximum eigenvalues of the Hessian of the validation loss for \text{DARTS} and the \text{UDARTS}, respectively, then \begin{equation}
\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})\leq \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) \nonumber
\end{equation}
\end{lemma}

These lemmas prove that the UDARTS architecture search method converges to a flatter minima for each iteration of the bi-level optimization. As discussed in the recent paper \cite{mulayoffunique}, flat minima implies that the gain from the input to any intermediate layer is well behaved. Furthermore, they also show that the consecutive layers in those solutions are coupled, forming a distinct path from input to output, which is dedicated to the signal that experiences the largest gain end-to-end.

==> tex/robustness_storage1.tex <==
\section{Robustness of UDARTS}
\label{sec:robust}
%Author et. al. has shown that the generalization performance of architectures found by the standard DARTS is related to the eigenvalues of the Hessian matrix of the validation loss with respect to  the architectural parameters. The standard DARTS often results in degenerate architectures with large eigenvalues and poor generalization. They showed using empirical results that properly regularizing the inner objective helps controlling the eigenvalue and therefore improves generalization. However, they used regularization as an addition to the early stopping mechanism which tracks the largest eigenvalue of the hessian of the validation loss at each time step. In this work, we prove that our proposed uncertainty based model search not only gives a model with low uncertainty, but also a more robust architecture, which is in accordance with our hypothesis that an architecture with low uncertainty will be more robust than the one with higher uncertainty.  

%Empirical results have shown that a generalization performance of the architecture found by DARTS improves with a lower eigenvalue of the Hessian matrix of the validation loss with respect to  the architectural parameters ($\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$). %improves the generalization performance of architectures found by the standard DARTS\cite{XX}.
%However, authors have used early stopping mechanism to limit the largest eigenvalue of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$. 
In this section, we prove that the eigenvalue of the Hessian of validation loss in UDARTS ($\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}}$) is lower than the eigenvalue of the Hessian of validation loss in DARTS ($\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$). %of the DARTS. %\textit{without using Hessian computation and early stopping}. %We assume the Hessian of the validation loss of DARTS and UDARTS with respect to the architecture parameters ($\alpha$) are given by $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ and $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}}$, respectively. 

%\subsection{Comparison with normal DARTS} 
\begin{comment}
Let us consider a neural network model with $L$ layers whose output is given as $\hat{\mathbf{y}}$ and a loss function $E(\cdot, \cdot)$ such as the softmax loss. We denote the NN's weight matrices as $\mathbf{W}_{i}$ and the bias vectors, $\mathbf{b}_{i}$ for each layer $i=1, \ldots, L .$ We denote by $\mathbf{y}_{i}$ the observed output corresponding to input $\mathbf{x}_{i}$ for $1 \leq i \leq N$ data points, and the input and output sets as $\mathbf{X}, \mathbf{Y}$. During NN optimisation a regularisation term is often added. We often use $L_{2}$ regularisation weighted by some weight decay $\lambda$, resulting in a minimisation objective (often referred to as cost),
\[\mathcal{L}_{\text {dropout }}:=\frac{1}{N} \sum_{i=1}^{N} E\left(\mathbf{y}_{i}, \widehat{\mathbf{y}}_{i}\right)+\lambda \sum_{i=1}^{L}\left(\left\|\mathbf{W}_{i}\right\|_{2}^{2}\right)\].

%Let's consider a neural network with $L$ layers where $l \in$ $\{0, \cdots, L-1\}$ is an index of the network layer. Index $l=0$ and $l=L-1$ are represented as the input layer and output layer, respectively. 
Suppose $\mathbf{z}^{(l)}$ denote the input vector to the layer $l$ and similarly, $\mathbf{y}^{(l)}$ express the output vector to the layer $l$.
%In addition, $\mathbf{W}^{(l)}$ and $\mathbf{b}^{(l)}$ are the weight and biased parameters at layer $l$. 
Based on the operation of the MLP network, the input and output vectors at the hidden layers $(l=1, \cdots, L-2)$ can be computed by:
\[
\begin{array}{l}
\mathbf{z}^{(l+1)}=\mathbf{W}^{(l+1)} \mathbf{y}^{(l)}+\mathbf{b}^{(l+1)} \\
\mathbf{y}^{(l+1)}=\mathbf{a}\left(\mathbf{z}^{(l+1)}\right)
\end{array}
\]
where $\mathbf{a}(.)$ is an activation function. When dropout is applied, the operation becomes:
\[
\begin{aligned}
\delta_{i}^{(l)} & \sim \operatorname{Bernoulli}(p) \\
\tilde{\mathbf{y}}^{(l)} &=\boldsymbol{\delta}^{(l)} \otimes \mathbf{y}^{(l)} \\
\mathbf{z}^{(l+1)} &=\mathbf{W}^{(l+1)} \tilde{\mathbf{y}}^{(l)}+\mathbf{b}^{(l+1)} \\
\mathbf{y}^{(l+1)} &=a\left(\mathbf{z}^{(l+1)}\right)
\end{aligned}
\]
where $\otimes$ is an element-by-element multiplication. $\delta_{i}^{(l)}$ is a Bernoulli random variable of neuron $i$ at layer $l$ with probability $\left(p_{i}\right)$ of being 1

Consider a dropout for a single linear unit (no hidden layer) with an input $x^{(i)} \in \mathbb{R}^{n} .$ The output can be calculated by a weighted sum of the input data.
\[
y^{(i)}=\sum_{k=1}^{n} w_{k} x_{k}^{(i)} \delta_{k}+b \delta_{b}
\]
\end{comment}

%Now, let us consider the Hessian of the validation loss given as $\nabla_{\alpha}^2 \mathcal{L}_{\text{valid}}$. 
%Since we are only interested in the largest eigenvalue, we can only concentrate on the local neighbourhood of the minima, which is convex in nature. Since the domain of our interest is convex, we can conclude that the Hessian is positive semi-definite and the eigenvalues are positive. 
%\\ Also, since the Hessian of our interest is $\nabla_{\alpha}^2 \mathcal{L}_{\text{valid}}$, we see that it is a diagonal matrix.
% Now, the spectral radius of the Hessian $\rho(A)$  is defined as  is the largest absolute value of its eigenvalues i.e., $\rho(A)=\max \left\{\left|\lambda_{1}\right|, \ldots,\left|\lambda_{n}\right|\right\}$ where $\lambda_i$ are the eigenvalues of the matrix $A$. 
% \\

%\textbf{Definitions.}
%We consider $\mathbf{x}_{i}$ is the input vector,  $\alpha$ is the weight matrix of architectural parameter, and $\mathbf{y}_i$ is the vector denoting the labels of the classes.


%\textbf{Definition 3.} The spectral radius of a matrix A   ($\rho(A)$)  is defined as  is the largest absolute value of its eigenvalues i.e., $\rho(A)=\max \left\{\left|\lambda_{1}\right|, \ldots,\left|\lambda_{n}\right|\right\}$ where $\lambda_i$ are the eigenvalues of the matrix $A$. 

% \begin{theorem}
% If $\rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}})$ and $\rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})$ be the spectral radii of the hessian of the standard \text{DARTS} and the \text{UDARTS} method respectively, then $\rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})\leq \rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}})$
% \label{th:robust}
% \end{theorem}

% \begin{proof}
% We prove the preceding theorem using following four Lemmas. 
% \end{proof}

% \begin{lemma}
% The validation loss function of the standard DARTS method is convex in nature.
% \label{lemma:convex}
% \end{lemma}

% \begin{proof}
% To prove that the cross entropy function is convex, we prove that \textit{the Hessian is positive semi-definite}. 

% For simplicity, we consider a linear model $\mathbf{x}_{i}^{T} \mathbf{\alpha}$, where $\mathbf{x}_{i}$ is the input vector and $\alpha$ is the weight matrix of architectural parameter. 
% Assume, $\mathbf{y}_i$ is the vector denoting the labels of the classes. Considering the cross entropy loss as the validation loss ($\mathcal{L}_{\text{valid}}$) we obtain:
% %Assume, $\mathbf{y}_i$ is the vector denoting the labels of the classes, $\mathbf{x}_{i}$ is the input vector and $\alpha$ is the weight matrix of architectural parameter. The hessian of the cross entropy loss is given as follows:
% \begin{equation}\mathcal{L}_{\text{valid}}^{\text{DARTS}}=-\frac{1}{N} \sum_{i=1}^{N} \mathbf{y}_{i} \log \left(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)+\left(1-\mathbf{y}_{i}\right) \log \left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)\end{equation}
% \begin{equation}\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}=\frac{1}{N} \sum_{i=1}^{N} \sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T}=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\mathbf{x}_{i} \mathbf{x}_{i}^{T}
% \end{equation}
% where, $\sigma(.)$ is the sigmoid function, and $\sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)$ for each $i$.

%  The Rayleigh quotient of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ is given by: 
% %the i.e., the smallest value taken by $\mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z}$
% %for any unit-length vector $\mathbf{z}$ and any possible weight vector $\mathbf{\alpha}$. 
% %Substituting in the particular form of the Hessian here, denoting $\sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)$ for each $i$ for short, we have
% \begin{equation}
% \mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z}=\mathbf{z}^{T}\left(\frac{1}{N} \sum_{i=1}^{N} \sigma_{i} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)\left(\mathbf{x}_{i}^{T} \mathbf{z}\right)=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2}
% \end{equation}
% where, $\mathbf{z}$ is any unit-length vector. %and any possible weight vector $\mathbf{\alpha}$. 
% We know that, the smallest eigenvalue of any square symmetric matrix is given as the minimum of the Rayleigh quotient of that matrix. Since $\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2} \geq 0$ and $\sigma_{i} \geq 0$, we must have $\mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z} \geq 0$. Consequently, the smallest possible eigenvalue of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ must be $\geq 0$. Hence, we conclude that the validation loss function ($\mathcal{L}_{\text{valid}}^{\text{DARTS}}$) is convex.
% % \end{proof}



% Since the validation loss of the standard DARTS( $\mathcal{L}_{\text{valid}}^{\text{DARTS}}$) is convex, the eigenvalues of the Hessian are strictly positive in nature. We know that if a matrix $A$ has positive eigenvalues then,   
% \begin{equation}\rho\left(A^{T} A\right) = \lambda_{\max }\left(A^{T} A\right) =\max _{x \neq 0} \frac{x^{T} A^{T} A x}{x^{T} x}=\max _{x \neq 0} \frac{\|A x\|_{2}^{2}}{\|x\|_{2}^{2}}= \|A\|_{2}^{2}\end{equation}.
\begin{lemma}
The largest eigenvalue of the Hessian of the validation loss of DARTS is given by, \[ \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = \frac{\max \sigma_i}{N}\lambda_{\max} (\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}) \text{, where, } \sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)\] %$\sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)$
\label{lemma:DARTS}
\end{lemma}



%\begin{proof}

\textit{Proof.} We consider $\mathbf{x}_{i}$ is the input vector,  $\alpha$ is the weight matrix of architectural parameter, and $\mathbf{y}_i$ is the vector denoting the labels of the classes.
For simplicity, we consider a linear model $\mathbf{x}_{i}^{T} \mathbf{\alpha}$ for this proof. %where $\mathbf{x}_{i}$ is the input vector and $\alpha$ is the weight matrix of architectural parameter. 
%Assume, $\mathbf{y}_i$ is the vector denoting the labels of the classes. 
Considering the cross entropy loss as the validation loss ($\mathcal{L}_{\text{valid}}$) we obtain:
%Assume, $\mathbf{y}_i$ is the vector denoting the labels of the classes, $\mathbf{x}_{i}$ is the input vector and $\alpha$ is the weight matrix of architectural parameter. The hessian of the cross entropy loss is given as follows:
\begin{equation}\mathcal{L}_{\text{valid}}^{\text{DARTS}}=-\frac{1}{N} \sum_{i=1}^{N} \mathbf{y}_{i} \log \left(\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)+\left(1-\mathbf{y}_{i}\right) \log \left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)\end{equation}
\begin{equation}\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}=\frac{1}{N} \sum_{i=1}^{N} \sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T}=\frac{1}{N} \sum_{i=1}^{N} \sigma_{d}\mathbf{x}_{i} \mathbf{x}_{i}^{T}
\end{equation}
where, $\sigma(.)$ is the sigmoid function, $\sigma_{d}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)$ for each $i$. %and $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ is the Hessian of the validation loss with respect to architectural parameters $\alpha$.
% As Hessian is a symmetric matrix, the largest eigenvalue of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}$ is given by maximum value of its  

We know the Rayleigh quotient of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ is given by: 
%the i.e., the smallest value taken by $\mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z}$
%for any unit-length vector $\mathbf{z}$ and any possible weight vector $\mathbf{\alpha}$. 
%Substituting in the particular form of the Hessian here, denoting $\sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)$ for each $i$ for short, we have
\begin{equation}
R_{DARTS}(\mathbf{z})=\mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z}=\mathbf{z}^{T}\left(\frac{1}{N} \sum_{i=1}^{N} \sigma_{d} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}=\frac{1}{N}\left(\mathbf{z}^{T}\left(\sum_{i=1}^{N} \sigma_{d}\mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}\right)
\label{eq:r_loss}
\end{equation}
where, $\mathbf{z}$ is any unit-length vector. Assuming maximum of $\sigma_{d}$ is represented as $\sigma_{d}^{max}$, we obtain:
\begin{equation}
R_{DARTS}(\mathbf{z}) \le \frac{\sigma_{d}^{max}}{N}\left(\mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}\right) = \frac{\sigma_{i}^{max}}{N}R_{M_{\mathbf{x}}}(\mathbf{z})
\end{equation}

% \begin{equation}
% R_{max}\left(\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}},\mathbf{z}\right) = \frac{\sigma_{max}}{N} max\left(\mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}\right)
% \label{eq:r_loss}
% \end{equation}
where, $R_{M}(\mathbf{z})$ is the Raleigh quotient of the matrix $M_{\mathbf{x}}=\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}$ as given by: 
\begin{equation}
R_{M}(\mathbf{z})=\mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}=\sum_{i=1}^{N} \left(\mathbf{z}^{T} \mathbf{x}_{i}\right)\left(\mathbf{x}_{i}^{T} \mathbf{z}\right)= \sum_{i=1}^{N} \left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2} \ge 0
\label{eq:r_sum}
\end{equation}


% \end{proof}


% \begin{equation}
% \mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z}=\mathbf{z}^{T}\left(\frac{1}{N} \sum_{i=1}^{N} \sigma_{i} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}
% \end{equation}


Since, the maximum eigenvalue of a symmetric matrix ($A$) is equal to the maximum value of its Raleigh quotient $\left(\lambda_{\max}(A)=R_{A}^{max})\right)$, we obtain: \begin{equation}
\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = R_{DARTS}^{\max}=\frac{ \sigma_{d}^{\max}}{N}R_{M
}^{\max}
=\frac{ \sigma_{d}^{\max}}{N} \lambda_{\max} \left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right)
\label{eq:spectral_DARTS}
\end{equation}
%\end{proof}

\textbf{Corollary.}  The validation loss function of the standard DARTS ($\mathcal{L}_{\text{valid}}^{\text{DARTS}}$) method is convex in nature.

\textbf{Proof.} We know that, the smallest eigenvalue of any square symmetric matrix is given as the minimum of the Rayleigh quotient of that matrix. Since $\sigma_{d} \geq 0$, from equations \ref{eq:r_loss} and \ref{eq:r_sum}, we obtain $R_{DARTS}(\mathbf{z}) \geq 0$. Hence, the smallest possible eigenvalue of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ must be zero or positive which implies that the validation loss function is convex.

% \begin{equation}
% \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = \frac{\max \sigma_i}{N}\max\left(\mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}\right)= \frac{\max \sigma_i}{N} \lambda_{\max} \left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right)
% \label{eq:spectral_DARTS}
% \end{equation}
% \end{proof}

% \begin{equation}
% R(\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}},\mathbf{z})=\mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z}=\mathbf{z}^{T}\left(\frac{1}{N} \sum_{i=1}^{N} \sigma_{i} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)\left(\mathbf{x}_{i}^{T} \mathbf{z}\right)=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2}
% \end{equation}

%and any possible weight vector $\mathbf{\alpha}$. 
%We know that, the smallest eigenvalue of any square symmetric matrix is given as the minimum of the Rayleigh quotient of that matrix. Since $\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2} \geq 0$ and $\sigma_{i} \geq 0$, we must have $\mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z} \geq 0$. Consequently, the smallest possible eigenvalue of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ must be $\geq 0$. Hence, we conclude that the validation loss function ($\mathcal{L}_{\text{valid}}^{\text{DARTS}}$) is convex.
% \end{proof}

%Building on the analysis above showing that the cross-entropy cost is convex, we can likewise compute its largest possible eigenvalue.
% We can evaluate the largest eigenvalue of $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}$ by calculating the largest value of its Rayleigh quotient for any $\mathbf{z}$ as shown below: %. . Thus the largest value the Rayleigh quotient can take is bounded above for any $\mathbf{z}$ as
% \begin{equation}
%     \mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z} \leq \frac{\max \sigma_i}{ N} \mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}
% \end{equation}

% Since the maximum value $\mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}$ can take is the maximum eigenvalue of the matrix $\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T},$ thus the maximum eigenvalue of the Hessian for the Cross Entropy loss function is given as
% \begin{equation}
% \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = \frac{\max \sigma_i}{N} \lambda_{\max} (\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T})
% \label{eq:spectral_DARTS}
% \end{equation}
% \end{proof}




















\begin{lemma}
The largest eigenvalue of the Hessian of the validation loss of UDARTS is given by, \[ \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}}) \le \frac{ \sigma_{ud}^{max}}{N}\lambda_{\text{max}}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \] 

\begin{flalign*} 
 \text{ where, } \sigma_{ud} &= \sqrt{\sigma_{x^2}}\left(1-\sqrt{\sigma_{x^2}}\right)  +  4\alpha^2 \sigma_{x^2}(1- \sigma_{x^2}) -8\alpha^2(\sigma_{x^2})^{2}(1- \sigma_{x^2}) \nonumber \\
 &- 2\sigma_{x^2}(1 - \sigma_{x^2}) -\frac{1}{2}\sqrt{\sigma_{x^2}}(1 - \sqrt{\sigma_{x^2}}) -0.1924 \sqrt{\sigma_{x^2}} \nonumber \\
 \sigma_{x^2} &= \sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) \text{ and } \sigma_{x} = \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})  \nonumber
\end{flalign*}



\label{lemma:UDARTS}
\end{lemma}


%\begin{proof}
%Building on the proof, we find the largest  eigenvalue of the standard DARTS by calculating the largest value the Rayleigh quotient. 
\textit{Proof.}To estimate $\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}}$, we add the predictive variance term to the DARTS validation loss. 
%If we consider that $\sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) \rightarrow \sigma_{x^2}$ and $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}) \rightarrow \sigma_{x}$
\begin{align}
&\operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) = \mathbb{E}((\mathbf{x}_{i}^{T}\alpha)^2)  - \mathbb{E}(\mathbf{x}^{T}_{i}\alpha)^2
= \frac{1}{T} \sum_{i=1}^{T}\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) - (\frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2} \\
&\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} = \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} +  \nabla_{\alpha}^{2} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) \nonumber\\
 &= \frac{1}{N} \sum_{i=1}^{N} \sigma_{x}\left(1-\sigma_{x}\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T} + \frac{1}{T} \sum_{i=1}^{T} \{ [\sigma_{x^2}(1- \sigma_{x^2}) -2\sigma_{x^2}^{2}(1- \sigma_{x^2})]4\alpha^{T}\alpha \mathbf{x}_{i}\mathbf{x}^{T}_{i} - \sigma_{x^2}(1 - \sigma_{x^2}) 2\mathbf{x}_{i}\mathbf{x}^{T}_{i} \} \nonumber\\ &- \frac{2}{T^{2}} [\sum_{i=1}^{T} \sigma_{x}(1- \sigma_{x})\sum_{i=1}^{T}\sigma_{x}(1- \sigma_{x})]\mathbf{x}_{i} \mathbf{x}_{i}^{T} -\frac{2}{T^{2}}[\sum_{i=1}^{T} \sigma_{x} \sum_{i=1}^{T} \sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})] \mathbf{x}_{i} \mathbf{x}_{i}^{T}
\end{align}
Without loss of generality, we consider the case when $T=N$. Therefore, the Raleigh quotients of $\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}}$ can be computed as: 

\begin{align}
&R_{UDARTS}(\mathbf{z})=\mathbf{z}^{T}\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} \mathbf{z} \nonumber \\
 &= \mathbf{z}^{T}\Bigg( \frac{1}{N}\sum_{i=1}^{N}
 \bigg[
 \sigma_{x}\left(1-\sigma_{x}\right)  +  \Big(\sigma_{x^2}(1- \sigma_{x^2}) -2\sigma_{x^2}^{2}(1- \sigma_{x^2})\Big)4\alpha^{T}\alpha - 2\sigma_{x^2}(1 - \sigma_{x^2}) 
 %\mathbf{x}_{i}\mathbf{x}^{T}_{i}  
 \nonumber \\ 
 %&- \frac{2}{N^2} \sum_{i=1}^{N} \sigma_{x}(1- \sigma_{x})\sum_{i=1}^{T}\sigma_{x}(1- \sigma_{x})]\mathbf{x}_{i} \mathbf{x}_{i}^{T} -\frac{2}{N^{2}}[\sum_{i=1}^{N} \sigma_{x} \sum_{i=1}^{N} \sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})]\right] \mathbf{x}_{i} \mathbf{x}_{i}^{T} \nonumbner \\
  %&- \frac{1}{N} \sum_{i=1}^{N}
  &- \frac{2}{N} \sigma_{x}(1- \sigma_{x})\sum_{i=1}^{N}\sigma_{x}(1- \sigma_{x}) -\frac{2}{N} \sigma_{x} \sum_{i=1}^{N} \Big(\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})\Big)\bigg] \mathbf{x}_{i}\mathbf{x}_{i}^{T}\Bigg)\mathbf{z} \nonumber \\
  &\implies R_{UDARTS}(z)= \mathbf{z}^{T}\Bigg( \frac{1}{N}\sum_{i=1}^{N}
 \bigg[\sigma_{j}\bigg]\mathbf{x}_{i}\mathbf{x}_{i}^{T}\Bigg)\mathbf{z} 
 %\le \frac{\sigma_{ud}^{\max}}{N}\Bigg(\mathbf{z}^{T}\bigg(\frac{1}{N}\sum_{i=1}^{N}
 %\mathbf{x}_{i}\mathbf{x}_{i}^{T}\bigg)\mathbf{z}\Bigg)
\end{align}


%Since the softmax is a convex function, we can use Jensen's inequality as $ \sigma_{x}^{2} \le \sigma_{x^2}$
where, $\sigma_{j}$ is the polynomial in $\sigma_x$, $\sigma_{x^2}$, and $\alpha$. We note that the following: 
\begin{align}
&\text{(i) } \sigma_{x}(1- \sigma_{x}) \leq \frac{1}{4}
\implies \sum_{i=1}^{T} \sigma_{x}(1- \sigma_{x}) \le  \sum_{i=1}^{T} \frac{1}{4} = \frac{T}{4} \nonumber \\
&\text{(ii) } [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})] \leq 0.0962 \implies \sum_{i=1}^{T} [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})] \le 0.0962T \nonumber
\end{align}

%maximum value of $\sigma_{x}(1- \sigma_{x})$ is $\frac{1}{4}$, so $\sum_{i=1}^{T} \sigma_{x}(1- \sigma_{x}) \le  \sum_{i=1}^{T} \frac{1}{4} = \frac{T}{4}$. Similarly, the maximum value of $ [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})]$ is given as $0.0962$. Therefore, $\sum_{i=1}^{T} [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})] \le 0.0962T$

Therefore, the polynomial $\sigma_{ud}$ satisfies the following inequalities: 
%the Raleigh quotients of $\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}}$ can be computed as: 
%\begin{align}
%\left
\begin{multline*}
\sigma_{j} 
\le  \Big[\sigma_{x}\left(1-\sigma_{x}\right)  + \Big(\sigma_{x^2}(1- \sigma_{x^2}) -2(\sigma_{x^2})^{2}(1- \sigma_{x^2})\Big)4\alpha^{T}\alpha \\
- 2\sigma_{x^2}(1 - \sigma_{x^2}) 
-\frac{1}{2} \sigma_{x}(1- \sigma_{x}) -0.1924 \sigma_{x}\Big] 
\end{multline*}
As $\sigma_{x}$ is convex, using Jensen's inequality ($\sigma_{x}^{2} \le \sigma_{x^2}$) we get:
\begin{multline*}
\sigma_{j}\le \Big[\sqrt{\sigma_{x^2}}\left(1-\sqrt{\sigma_{x^2}}\right)  + 4\alpha^2\sigma_{x^2}(1- \sigma_{x^2}) -8\alpha^2(\sigma_{x^2})^{2}(1- \sigma_{x^2}) \\
- 2\sigma_{x^2}(1 - \sigma_{x^2})  
-\frac{1}{2} \sqrt{\sigma_{x^2}}(1 - \sqrt{\sigma_{x^2}}) -0.1924 \sqrt{\sigma_{x^2}}\Big] = \sigma_{ud}
% \le  \frac{1}{T} \sum_{i=1}^{T} [\sqrt{\sigma_{x^2}}\left(1-\sqrt{\sigma_{x^2}}\right)  +  4\alpha^2 \sigma_{x^2}(1- \sigma_{x^2}) -8\alpha^2(\sigma_{x^2})^{2}(1- \sigma_{x^2}) \\
% - 2\sigma_{x^2}(1 - \sigma_{x^2}) -\frac{1}{2}\sqrt{\sigma_{x^2}}(1 - \sqrt{\sigma_{x^2}}) -0.1924 \sqrt{\sigma_{x^2}} ] (\mathbf{z}^{T} \mathbf{x}_{i})^2 
\end{multline*}
Assuming, maximum value of $\sigma_{ud}$ and $\sigma_{j}$ are given by $\sigma_{ud}^{\max}$ and $\sigma_{j}^{\max}$, respectively, we obtain:
\begin{equation}
 R_{UDARTS}(z) 
 \le \frac{\sigma_{j}^{\max}}{N}\Bigg(\mathbf{z}^{T}\Bigg(\sum_{i=1}^{N}
\mathbf{x}_{i}\mathbf{x}_{i}^{T}\Bigg)\mathbf{z}\Bigg)
 \le \frac{\sigma_{ud}^{\max}}{N}\Bigg(\mathbf{z}^{T}\Bigg(\sum_{i=1}^{N}
\mathbf{x}_{i}\mathbf{x}_{i}^{T}\Bigg)\mathbf{z}\Bigg)
 \end{equation}
%ubstituting  $\sigma_j$ in the above we obtain: 
% \begin{equation}
% \mathbf{z}^{T}\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} \mathbf{z}  \le  \frac{1}{N} \sum_{i=1}^{N} \sigma_j (\mathbf{z}^{T} \mathbf{x}_{i})^2 
% \end{equation}
%\left
%\end{align}
%where $\sigma_j = \sqrt{\sigma_{x^2}}\left(1-\sqrt{\sigma_{x^2}}\right)  +  4\alpha^2 \sigma_{x^2}(1- \sigma_{x^2}) -8\alpha^2(\sigma_{x^2})^{2}(1- \sigma_{x^2}) - 2\sigma_{x^2}(1 - \sigma_{x^2}) -\frac{1}{2}\sqrt{\sigma_{x^2}}(1 - \sqrt{\sigma_{x^2}}) -0.1924 \sqrt{\sigma_{x^2}} $
Using the relation between maximum eigenvalue and Ralyeigh quotient, similar to the Lemma \ref{lemma:DARTS}, the largest eigenvalue of the UDARTS method is given as:
\begin{equation}
\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = R_{UDARTS}^{\max} \le \frac{ \sigma_{ud}^{\max}}{N} \lambda_{\max} \left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right)
\label{eq:spectral_UDARTS}
\end{equation}


% \begin{equation}
% \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}}) = \frac{\max \sigma_j}{N}R_{\max}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T},\mathbf{z}\right)=\frac{\max \sigma_j}{N}\lambda_{\text{max}}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right)
% \label{eq:spectral_UDARTS}
% \end{equation}
%\end{proof}

\begin{lemma}
If $\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}})$ and $\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})$ be the maximum eigenvalues of the Hessian of the validation loss for \text{DARTS} and the \text{UDARTS}, respectively, then \begin{equation}
\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})\leq \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) \nonumber
\end{equation}
\end{lemma}

%\begin{proof}


%Treating this equation as a polynomial in $\sigma_{x^2}$ such that the values of $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}) \in [0,1]$,


\textit{Proof.} We represent $\sigma_{d}$ as: 
$\sigma_{d} = p(1-p)$, where $p=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right) \in [0,1]$ due to the properties of the sigmoid function. Moreover, since $\alpha$ is the weights in the neural network we have $\alpha < 1 \implies \alpha^2 < 1$. Hence, by maximizing $\sigma_i$ with respect to $p$ we obtain:$\sigma_{d}^{\max} = 0.25$

We now represent $\sigma_{ud} = \frac{1}{2} \sqrt{q}(1-\sqrt{q})+4\alpha^2[ q(1-q)- 2q^{2}(1-q)]-2 q(1-q)-0.1924 \sqrt{q}$, where $q=\sigma_{{x}^2} = \sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) \in [0,1] $. We now maximize $\sigma_j$ with respect to $q$. At $q= 0.1132$, the function achieves the maximum value. Finally, noting $\alpha^2  < 1$, we obtain  
\begin{equation}
\sigma_{ud}^{\max} = [(0.310634)\alpha^2 -0.15388] < 0.16 < 0.25 = \sigma_{d}^{max} 
\label{eq:sigma}
\end{equation}

From equation (\ref{eq:r_sum}) we note that $R_{M}^{max} \geq 0$. Therefore, using equations  (\ref{eq:spectral_DARTS}), (\ref{eq:spectral_UDARTS}), and (\ref{eq:sigma}), we get
\begin{equation}
\lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})\leq \lambda_{\text{max}}(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}})
\end{equation}
Hence, we prove that maximum eigenvalue of Hessian of the validation loss of  UDARTS is smaller than that of DARTS.  

 %Since sigmoid function $\sigma$ is represented as $x$, the domain of our function is $[0,1]$. Thus, the maximum value of the polynomial is  achieved at $x= 0.1132$ when it reached the value $(0.310634)\alpha^2 -0.15388$> Thus, we can see that $\max \sigma_j \le \sigma_i$ for $\alpha^2 < 1.3$.  Since $\alpha$ is the weights in the neural network, $\alpha < 1 \Rightarrow \alpha^2 < 1$. Hence, the maximum value of the function is always lesser than the maximum value of the standard DARTS method.
%\end{proof}

\begin{comment}

\textbf{Proof:} 
We are using the cross entropy loss as the  validation loss function, $\mathcal{L}_{\text{valid}}$. If $\mathbf{y}_i$ is the vector denoting the labels of the classes, $\mathbf{x}_{i}$ is the input vector and $\alpha$ is the weight matrix , the gradient and the corresponding Hessian of the cross entropy loss are given as follows:
\begin{equation}\mathcal{L}_{\text{valid}}^{\text{DARTS}}=-\frac{1}{N} \sum_{i=1}^{N} \mathbf{y}_{i} \log \left(\sigma\left(\texttt{model}\left(\mathbf{x}_{i}, \mathbf{\alpha}\right)\right)\right)+\left(1-\mathbf{y}_{i}\right) \log \left(1-\sigma\left(\texttt{model}\left(\mathbf{x}_{i}, \mathbf{\alpha}\right)\right)\right)\end{equation}

For this proof we consider a linear model given as $\texttt{model}\left(\mathbf{x}_{i}, \mathbf{\alpha}\right)=\mathbf{x}_{i}^{T} \mathbf{\alpha}$
\begin{equation}\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}=\frac{1}{N} \sum_{i=1}^{N} \sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T}\end{equation}
We know that the largest eigenvalue of any square symmetric matrix is given as the maximum of the Rayleigh quotient, i.e., the largest value taken by
$\mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}} \mathbf{z}$
for any unit-length vector $\mathbf{z}$ and any possible weight vector $\mathbf{\alpha}$. Substituting in the particular form of the Hessian here, denoting $\sigma_{i}=\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)$ for each $i$ for short, we have
\begin{equation}
\mathbf{z}^{T} (\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{DARTS}}) \mathbf{z}=\mathbf{z}^{T}\left(\frac{1}{N} \sum_{i=1}^{N} \sigma_{i} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)\left(\mathbf{x}_{i}^{T} \mathbf{z}\right)=\frac{1}{N} \sum_{i=1}^{N} \sigma_{i}\left(\mathbf{z}^{T} \mathbf{x}_{i}\right)^{2}
\end{equation}



Since the largest eigenvalue is given by the largest value the Rayleigh quotient can take, it is bounded above for any $\mathbf{z}$ as
\begin{equation}
    \mathbf{z}^{T} \nabla_{\alpha}^{2} g(\mathbf{\alpha}) \mathbf{z} \leq \frac{\max \sigma_i}{ N} \mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}
\end{equation}
Again, since the maximum value $\mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}$ can take is the maximum eigenvalue of the matrix $\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T},$ thus the spectral radius for the Cross Entropy cost is given as
\begin{equation}
\rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = \frac{\max \sigma_i}{N}\left\|\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right\|_{2}^{2}
\end{equation}

For the UDARTS method,
\begin{align}
\operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) &= \mathbb{E}((\mathbf{x}_{i}^{T}\alpha)^2)  - \mathbb{E}(\mathbf{x}^{T}_{i}\alpha)^2
= \frac{1}{T} \sum_{i=1}^{T}\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) - (\frac{1}{T} \sum_{i=1}^{T}\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}))^{2} = \\
\nabla_{\alpha}^{2} \operatorname{Var}_{p(\mathbf{y} | \mathbf{x})}^{model}(\mathbf{\alpha}) 
&= \frac{1}{T} \sum_{i=1}^{T} \{ [\sigma_{x^2}(1- \sigma_{x^2}) -2\sigma_{x^2}^{2}(1- \sigma_{x^2})]4\alpha^{T}\alpha \mathbf{x}_{i}\mathbf{x}^{T}_{i} + \sigma_{x^2}(1 - \sigma_{x^2}) 2\mathbf{x}_{i}\mathbf{x}^{T}_{i} \} \nonumber\\ &- \frac{2}{T^{2}} \sum_{i=1}^{T} \sigma_{x}(1- \sigma_{x})\sum_{i=1}^{T}\sigma_{x}(1- \sigma_{x}) -\frac{2}{T^{2}}\sum_{i=1}^{T} \sigma_{x} \sum_{i=1}^{T} [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})] \mathbf{x}_{i} \mathbf{x}_{i}^{T}
\end{align}

Thus, the Hessian is given as:
\begin{align}
    \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} &= \frac{1}{N} \sum_{i=1}^{N} \sigma_{x}\left(1-\sigma_{x}\right) \mathbf{x}_{i} \mathbf{x}_{i}^{T} + \frac{1}{T} \sum_{i=1}^{T} \{ [\sigma_{x^2}(1- \sigma_{x^2}) -2\sigma_{x^2}^{2}(1- \sigma_{x^2})]4\alpha^{T}\alpha \mathbf{x}_{i}\mathbf{x}^{T}_{i} + \sigma_{x^2}(1 - \sigma_{x^2}) 2\mathbf{x}_{i}\mathbf{x}^{T}_{i} \} \nonumber\\ &- \frac{2}{T^{2}} \sum_{i=1}^{T} \sigma_{x}(1- \sigma_{x})\sum_{i=1}^{T}\sigma_{x}(1- \sigma_{x}) -\frac{2}{T^{2}}\sum_{i=1}^{T} \sigma_{x} \sum_{i=1}^{T} [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})] \mathbf{x}_{i} \mathbf{x}_{i}^{T}
\end{align}

where we consider that $\sigma(\mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}) \rightarrow \sigma_{x^2}$ and $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}) \rightarrow \sigma_{x}$.

Since we can choose the number of samples $T$, without loss of generality, let us consider the case when $T=N$.
Again, since the softmax is a convex function, we can use Jensen's inequality as $ \sigma_{x}^{2} \le \sigma_{x^2}$
Also, we note that the maximum value of $\sigma_{x}(1- \sigma_{x})$ is $\frac{1}{4}$, so $\sum_{i=1}^{T} \sigma_{x}(1- \sigma_{x}) \le  \sum_{i=1}^{T} \frac{1}{4} = \frac{T}{4}$. Similarly, the maximum value of $ [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})]$ is given as $0.0962$. Therefore, $\sum_{i=1}^{T} [\sigma_{x}(1- \sigma_{x}) -2(\sigma_{x})^2(1-\sigma_{x})] \le 0.0962T$

Therefore the Hessian simplifies to the following form:
\begin{align}
\nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}} 
% &\le  \frac{1}{T} \sum_{i=1}^{T} [\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\left(1-\sigma\left(\mathbf{x}_{i}^{T} \mathbf{\alpha}\right)\right)  + \nonumber \\ & \{ [4\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -8(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))]\alpha^{T}\alpha \nonumber\\ &+ 2\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))  \} \nonumber\\ &-\frac{1}{2} \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})(1- \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})) -0.1924 \sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha})] \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
&\le  \frac{1}{T} \sum_{i=1}^{T} [\sigma_{x}\left(1-\sigma_{x}\right)  + \{ [4\sigma_{x^2}(1- \sigma_{x^2}) -8(\sigma_{x^2})^{2}(1- \sigma_{x^2})]\alpha^{T}\alpha \nonumber\\ &- 2\sigma_{x^2}(1 - \sigma_{x^2})  \} -\frac{1}{2} \sigma_{x}(1- \sigma_{x}) -0.1924 \sigma_{x}] \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
%  &\le  \frac{1}{T} \sum_{i=1}^{T} [\sqrt{\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})}\left(1-\sqrt{\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})}\right)  + \nonumber\\ & 4\alpha^2 \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) -8\alpha^2(\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))^{2}(1- \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T}))] \nonumber\\&+ 2\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})(1 - \sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})) \nonumber\\ &-\frac{1}{2}\sqrt{\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})}(1 - \sqrt{\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})}) -0.1924 \sqrt{\sigma( \mathbf{\alpha} \mathbf{x}_{i} \mathbf{x}_{i}^{T} \mathbf{\alpha}^{T})} ] \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
 &\le  \frac{1}{T} \sum_{i=1}^{T} [\sqrt{\sigma_{x^2}}\left(1-\sqrt{\sigma_{x^2}}\right)  +  4\alpha^2 \sigma_{x^2}(1- \sigma_{x^2}) -8\alpha^2(\sigma_{x^2})^{2}(1- \sigma_{x^2}) \nonumber\\&- 2\sigma_{x^2}(1 - \sigma_{x^2}) -\frac{1}{2}\sqrt{\sigma_{x^2}}(1 - \sqrt{\sigma_{x^2}}) -0.1924 \sqrt{\sigma_{x^2}} ] \mathbf{x}_{i} \mathbf{x}_{i}^{T} \\
    \Rightarrow \mathbf{z}^{T} \nabla_{\alpha}^{2} \mathcal{L}_{\text{valid}}^{\text{UDARTS}}  \mathbf{z} &\leq \frac{\max \sigma_j}{ N} \mathbf{z}^{T}\left(\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right) \mathbf{z}
\end{align}

where $\sigma_j = \sqrt{\sigma_{x^2}}\left(1-\sqrt{\sigma_{x^2}}\right)  +  4\alpha^2 \sigma_{x^2}(1- \sigma_{x^2}) -8\alpha^2(\sigma_{x^2})^{2}(1- \sigma_{x^2}) - 2\sigma_{x^2}(1 - \sigma_{x^2}) -\frac{1}{2}\sqrt{\sigma_{x^2}}(1 - \sqrt{\sigma_{x^2}}) -0.1924 \sqrt{\sigma_{x^2}} $

Therefore, the spectral radius of the UDARTS method is given as:
\begin{equation}
\rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}}) = \frac{\max \sigma_j}{N}\left\|\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right\|_{2}^{2}
\end{equation}

% We know that the spectral radius of the normal DARTS method is given as 
% \begin{equation}
% \rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}}) = \frac{\max \sigma_{x}\left(1-\sigma_{x}\right)}{ N}\left\|\sum_{i=1}^{N} \mathbf{x}_{i} \mathbf{x}_{i}^{T}\right\|_{2}^{2}.
% \end{equation}

Treating this equation as a polynomial in $\sigma_{x^2}$ such that the values of $\sigma(\mathbf{x}_{i}^{T} \mathbf{\alpha}) \in [0,1]$, we get the following polynomial: $f(x) = \frac{1}{2} \sqrt{x}(1-\sqrt{x})+4\alpha^2[ x(1-x)- 2x^{2}(1-x)]-2 x(1-x)-0.1924 \sqrt{x}$. Now, since sigmoid function $\sigma$ is represented as $x$, the domain of our function is $[0,1]$. Thus, the maximum value of the polynomial is  achieved at $x= 0.1132$ when it reached the value $(0.310634)\alpha^2 -0.15388$> Thus, we can see that $\max f(x) \le \frac{1}{4}$ for $\alpha^2 < 1.3$.  Since $\alpha$ is the weights in the neural network, $\alpha < 1 \Rightarrow \alpha^2 < 1$. Hence, the maximum value of the function is always lesser than the maximum value of the standard DARTS method.

 

Hence we may say that the spectral radius of the Hessian of the UDARTS are smaller than the ones of the DARTS method. Therefore, 
\[\rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{DARTS}})  \ge \rho(\nabla_{\alpha}^{2}\mathcal{L}_{\text{valid}}^{\text{UDARTS}})  \]



\end{comment}





%We conclude that maximum eigenvalue of Hessian of the validation loss of  UDARTS is smaller than that of DARTS. This implies that the architectural search in UDARTS converges to a flatter minima and is more stable compared to the other methods. Also, unlike RobustDARTS, the proposed UDARTS method does not use Hessian computation and early stopping during architecture search to converge in a flatter minima resulting in a faster computation.


